On the Equivalence between Positional Node Embeddings and Structural Graph Representations

This work provides the first unifying theoretical framework for node (positional) embeddings and structural graph representations, bridging methods like matrix factorization and graph neural networks. Using invariant theory, we show that the relationship between structural representations and node embeddings is analogous to that of a distribution and its samples. We prove that all tasks that can be performed by node embeddings can also be performed by structural representations and vice-versa. We also show that the concept of transductive and inductive learning is unrelated to node embeddings and graph representations, clearing another source of confusion in the literature. Finally, we introduce new practical guidelines to generating and using node embeddings, which fixes significant shortcomings of standard operating procedures used today.

==> section_tex_files/experimental_outline.tex <==
\subsection{Model}
The colliders model will be used for all of the following tasks to get positional embeddings. An expectation over a function of the pos embeddings will be used to get the structural embeddings of the node / node set. Structural embeddings of the node / node set are then used to make predictions.

\subsection{Objective for positional samples}
Will use two objectives to generate positional embeddings
\begin{itemize}
    \item Predict links between pairs of nodes
    \item Predict triads (not traingles) between triplets of nodes. (Note: Will assume a random ordering of the nodes in every epoch)
\end{itemize}

\subsection{Tasks with Structural Embeddings}
Will use the structural embeddings to predict the following, irrespective of which objective was used to generate the positional embeddings.
Have included datasets in paranthesis.
\begin{itemize}
    \item Node Classification (Cora, Citeseer, Pubmed)
    \item Link Prediction (Cora, Citeseer, Pubmed, UW-CSE) Metric - Accuracy, AUC-PR to compare with Le Song's work
    \item Triad Prediction (Cora, Citeseer, Pubmed)
    \item Graph Classification (CSL task from RP)
\end{itemize}
Will add Reddit and some more graph classification tasks, time permitting

==> section_tex_files/model.tex <==
%The true model
%Write about our model as well as the others model
%Justify our model and say how the other model doesn't capture edge dependencies
%Justify why the other model is what other models are actually doing because they dont have a colliders in place
\begin{comment}


Edges are not independent of each other in a real world graph. The most powerful/ expressive model should therefore capture this. 

\begin{figure}[H]
	\begin{center}
        \includegraphics[scale=0.7]{figures/graph_data.pdf}
		\vspace{-10pt}
	\end{center}
	\caption{Data}
	\label{fig:model_data}
	\vspace{-1.8em}
\end{figure}

\begin{figure}[H]
	\begin{center}
        \includegraphics[scale=0.7]{figures/graph_model.pdf}
		\vspace{-10pt}
	\end{center}
	\caption{Powerful model}
	\label{fig:model_model}
	\vspace{-1.8em}
\end{figure}

The model is constructed as follows:
\begin{enumerate}
    \item A RV $x_i$ is introduced for every node $i \in V$, we note that these are observed
    \item A RV $e_{ij}$ is introduced for every pair of nodes $i,j  \in V, i \neq j$ - this represents the edges and the non edges. Again, if the edges are present in the original graph - they are observed
    \item A RV $y_i$ is introduced for every node $i \in V$, these are unobserved
\end{enumerate}

We make edges in the graphical model as follows:
\begin{enumerate}
    \item Every $x_i$ is connected to every $y_i$
    \item Every $e_{ij}$ is connected to every $y_i$
    \item Every $y_i$ is connected to every other $y_j$
\end{enumerate}
\end{comment}


\begin{comment}
Structure of the model: Model Roll Out
\begin{enumerate}
    \item Random variable is introduced for every node in the graph as well as for every edge
    \item latent variables as well
    \item clique template - all latent variables are connected
\end{enumerate}
\end{comment}
